Molecular Nature of Thermodynamics and its Application to Nanosize Particle Systems

The origins of thermodynamics from the microscopic properties of matter have not been satisfactorily accounted for. This work presents a formulation that connects Lagrangian mechanics to thermodynamics. By using such a formulation and following similar steps to those performed in the laboratory, the heat capacities, energetic and mechanical response coefficients, absorbed and emitted heats, entropy changes, and thermodynamic energies of a prototype water system, employed as an illustrative example, are found to be close to the experimental results on water bulk. The present formulation is realistic. After connecting Lagrangian mechanics to Langevin stochastic dynamics, the first law of thermodynamics is derived. The formulation not only exhibits the transformation of time-reversible equations onto time-irreversible equations, and the molecular origins of heat as well, but also reveals new pathways to investigate the thermodynamics of systems of nanometric sizes.

==> plot/data/energy-vol.tex <==



==> plot/data/fig02-ent1.tex <==



==> plot/data/fig02-ent2.tex <==



==> plot/data/fig02-ent3.tex <==



==> plot/data/fig02-temp.tex <==



==> plot/data/vconf-temp.tex <==



==> plot/data/vol-rho.tex <==


